RipBench: A Unified Benchmark for Multi-Level Rip Current Detection, Classification and Segmentation

Rip currents are a serious and often under-addressed threat to beach safety and the leading cause of coastal drownings worldwide. They are difficult to detect due to their amorphous structure, similarity to the background, and large variability in viewpoints and environments. Despite their dangers and growing interest in automated detection, existing research remains fragmented across datasets, metrics, models, and approaches, leading to an incomplete understanding of model performance. We introduce RipBench, a unified benchmark that enables controlled evaluation of rip current detection spanning multiple tasks, including classification, axis-aligned and oriented object detection, and instance, semantic, and panoptic segmentation, on the same data with standardized splits. This allows direct comparison of model performance on all levels of visual abstraction. Across $304$ videos ($303{,}491$ frames, $51{,}011$ of them annotated for all six tasks) collected from diverse coastlines, our results expose a clear performance gap between coarse recognition and precise spatial understanding: frame-level classification reaches $F_2 = 0.93$, while the best detector and the best instance segmenter reach $0.72$ and $0.66$, with model rankings that change from task to task. Video-level confidence intervals, a blind inter-annotator study of the spatial labels, stratified analyses by viewpoint and visual signature, and video views with temporal baselines (single-seed, short-schedule reference runs) accompany the benchmark. All tasks are supported with carefully curated annotations and evaluated using standard metrics, with a focus on the $F_2$ score to emphasize recall in this safety-critical setting. RipBench, along with multiple baselines per task, is publicly available at https://RipBench.ai to support progress in real-world, multi-task vision for beach safety.

==> tables/obb_full.tex <==
\begin{table}[!htbp]
  \caption{Oriented detection on the test split (rotated-polygon IoU $0.50$). $F_2$ with its 95\% video-level CI, best in \textcolor{blue}{blue}; canonical training scenario, protocol in Sec.~\ref{sec:eval_protocol}.}
  \label{tab:obb-detection-full}
  \centering
  \small
  \fittable{\begin{tabular}{lcccccc}
    \toprule
    Model & $AP_{50}$ & P & R & $F_1$ & $F_2$ [95\% CI] & FPS \\
    \midrule
    YOLO26-n & 0.379 & 0.491 & 0.432 & 0.460 & 0.443 [0.16, 0.64] & 251 \\
    YOLO26-s & 0.329 & 0.439 & 0.401 & 0.419 & 0.408 [0.15, 0.63] & 244 \\
    YOLO26-m & 0.367 & 0.430 & 0.442 & 0.436 & 0.439 [0.18, 0.63] & 229 \\
    YOLO26-l & 0.388 & 0.508 & 0.451 & 0.478 & \textcolor{blue}{0.462} [0.23, 0.66] & 178 \\
    YOLO26-x & 0.376 & 0.455 & 0.441 & 0.448 & 0.444 [0.18, 0.65] & 154 \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tables/panoptic.tex <==
\begin{table}[!htbp]
  \caption{Panoptic segmentation on the test split (COCO panoptic protocol; rip current is the only thing class, so $PQ_{rip}=PQ_{th}$; background = water/land/sky); $PQ_{rip}$ with its 95\% video-level CI, best in \textcolor{blue}{blue}; canonical training scenario.}
  \label{tab:pan-segmentation}
  \centering
  \small
  \fittable{\begin{tabular}{lccccccc}
    \toprule
    Model & $PQ_{rip}$ [95\% CI] & $SQ_{rip}$ & $RQ_{rip}$ & $PQ_{bg}$ & $RQ_{bg}$ & $PQ$ & FPS \\
    \midrule
    Mask2Former-R50 & 0.396 [0.21, 0.52] & 0.696 & 0.568 & 0.943 & 0.990 & 0.806 & 41 \\
    Mask2Former-Swin-L & \textcolor{blue}{0.465} [0.27, 0.58] & 0.695 & 0.670 & 0.946 & 0.985 & 0.826 & 23 \\
    MaskDINO-Swin-L & 0.459 [0.25, 0.58] & 0.695 & 0.661 & 0.947 & 0.985 & 0.825 & 17 \\
    \bottomrule
  \end{tabular}}
\end{table}


==> tables/panoptic_full.tex <==



==> tables/semantic.tex <==
\begin{table}[!htbp]
  \caption{Semantic segmentation on the test split: per-class IoU and pixel-level $F$-scores (rip class and mean over water/land/sky); rip IoU with its 95\% video-level CI, best in \textcolor{blue}{blue}; canonical training scenario.}
  \label{tab:semantic-segmentation}
  \centering
  \small
  \fittable{\begin{tabular}{lcccccccc}
    \toprule
    Model & $IoU_{rip}$ [95\% CI] & $mIoU_{bg}$ & ${F_1}_{rip}$ & ${F_2}_{rip}$ & ${F_1}_{bg}$ & ${F_2}_{bg}$ & Pixel acc. & FPS \\
    \midrule
    Mask2Former-R50 & 0.376 [0.18, 0.50] & 0.967 & 0.547 & 0.506 & 0.983 & 0.984 & 0.969 & 31 \\
    MaskDINO-R50 & 0.397 [0.19, 0.52] & 0.969 & 0.568 & 0.519 & 0.984 & 0.986 & 0.972 & 31 \\
    YOLO26-n & \textcolor{blue}{0.406} [0.16, 0.55] & 0.955 & 0.577 & 0.508 & 0.977 & 0.978 & 0.964 & 423 \\
    YOLO26-s & 0.342 [0.13, 0.48] & 0.958 & 0.510 & 0.436 & 0.978 & 0.980 & 0.965 & 426 \\
    YOLO26-m & 0.379 [0.15, 0.51] & 0.965 & 0.550 & 0.468 & 0.982 & 0.984 & 0.970 & 362 \\
    YOLO26-l & 0.395 [0.18, 0.53] & 0.964 & 0.567 & 0.501 & 0.982 & 0.983 & 0.969 & 265 \\
    YOLO26-x & 0.387 [0.17, 0.51] & 0.960 & 0.558 & 0.481 & 0.980 & 0.981 & 0.967 & 216 \\
    \bottomrule
  \end{tabular}}
  \\[2pt] {\footnotesize Validation-selected configuration where it differs from the family-best row shown (test value): MaskDINO-R50 (rip-IoU-selected) 0.375.}
\end{table}


==> tables/semantic_full.tex <==


